A large family of indecomposable projective modules for the Khovanov-Kuperberg algebra of $sl_3$-webs

We recall a construction of Mackaay, Pan and Tubbenhauer of the algebras $K^{\epsilon}$ which allow to understand the $sl_3$ homology for links in a local way (i.e. for tangles). Then, by studying the combinatorics of the Kuperberg bracket, we give a large family of non-elliptic webs whose associated projective $K^{\epsilon}$-modules are indecomposable.

==> sw_ex_conjugate.tex <==
\begin{scope}[xshift = 0cm, yscale = {1}, xscale={1},decoration={markings, mark=at
     position 0.5 with {\arrow{>}}},postaction={decorate}]
\coordinate [label=below:{$+$}] (A) at (0,0);
\coordinate [label=below:{$+$}] (B) at (1,0);
\coordinate [label=below:{$+$}] (C) at (2,0);
\coordinate [label=above:{$+$}] (D) at (0,4);
\coordinate [label=above:{$+$}] (E) at (1,4);
\coordinate [label=above:{$-$}] (F) at (2,4);
\coordinate [label=above:{$-$}] (G) at (3,4);
\draw[postaction=decorate] (A) -- (D);
\draw[postaction=decorate] (B) -- (E);
\draw[postaction=decorate] (C) .. controls (2,1) and (2.5,2) .. (2.5,2.5);
\draw[postaction=decorate] (G) .. controls (3,3) and (3,3) .. (2.5,2.5);
\draw[postaction=decorate] (F) .. controls (2,3) and (2,3) .. (2.5,2.5);
\end{scope}

\begin{scope}[xshift = 9cm, yshift =  4cm, yscale = {-1}, xscale={1},decoration={markings, mark=at
     position 0.5 with {\arrow{<}}},postaction={decorate}]
\coordinate [label=above:{$+$}] (A) at (0,0);
\coordinate [label=above:{$+$}] (B) at (1,0);
\coordinate [label=above:{$+$}] (C) at (2,0);
\coordinate [label=below:{$+$}] (D) at (0,4);
\coordinate [label=below:{$+$}] (E) at (1,4);
\coordinate [label=below:{$-$}] (F) at (2,4);
\coordinate [label=below:{$-$}] (G) at (3,4);
\draw[postaction=decorate] (A) -- (D);
\draw[postaction=decorate] (B) -- (E);
\draw[postaction=decorate] (C) .. controls (2,1) and (2.5,2) .. (2.5,2.5);
\draw[postaction=decorate] (G) .. controls (3,3) and (3,3) .. (2.5,2.5);
\draw[postaction=decorate] (F) .. controls (2,3) and (2,3) .. (2.5,2.5);
\end{scope}

==> sw_semi_superficial.tex <==
\begin{scope}[yscale ={0.6}, xscale={1},decoration={markings, mark=at
     position 0.5 with {\arrow{>}}},postaction={decorate}]
      \draw[dotted] (1.5,1.5) circle (1.414 cm);
      %\draw[postaction = {decorate}] (0,0)--(3,0); an Hexagon and 
      \draw[postaction = {decorate}] (0.5,0.5)--(1,1);
      %\draw[postaction = {decorate}] (0,0)--(0,3);
      %\draw[postaction = {decorate}] (3,3)--(0,3);
      \draw[postaction = {decorate}] (2,2) -- (2.5,2.5);
      \draw[postaction = {decorate}] (1.5,1)--(1.5,2);
      \draw[postaction = {decorate}] (1.5,1)--(1,1);
      \draw[postaction = {decorate}] (1.5,1)--(2,1);
      \draw[postaction = {decorate}] (2,2)--(2,1);
      \draw[postaction = {decorate}] (2.5,0.5) -- (2,1);
      \draw[postaction = {decorate}] (2,2) -- (1.5,2);
      \draw[postaction = {decorate}] (1,2) -- (1.5,2);
      \draw[postaction = {decorate}] (1,2)--(1,1);
      \draw[postaction = {decorate}] (1,2)--(0.5,2.5);
      \node at (1.5,0.4) {$C$};
      \node at (1.25,1.5) {$S_1$};
      \node at (1.75,1.5) {$S_2$};
      \node at (1.5,2.6) {$A$};
      \node at (0.4,1.5) {$D$};
%      \node at (1.5,1.5) {$C$};
      \node at (2.6,1.5) {$B$};
 \end{scope}

==> sw_square-notation.tex <==
\begin{scope}[scale={1},decoration={markings, mark=at
     position 0.5 with {\arrow{>}}},postaction={decorate}]
      \draw[dotted] (1.5,1.5) circle (1.414 cm);
      %\draw[postaction = {decorate}] (0,0)--(3,0);
      \draw[postaction = {decorate}] (0.5,0.5)--(1,1);
      %\draw[postaction = {decorate}] (0,0)--(0,3);
      %\draw[postaction = {decorate}] (3,3)--(0,3);
      \draw[postaction = {decorate}] (2.5,2.5)--(2,2);
      %\draw[postaction = {decorate}] (3,3)--(3,0);
      \draw[postaction = {decorate}] (2,1)--(1,1);
      \draw[postaction = {decorate}] (2,1)--(2,2);
      \draw[postaction = {decorate}] (2,1)--(2.5,0.5);
      \draw[postaction = {decorate}] (1,2)--(2,2);
      \draw[postaction = {decorate}] (1,2)--(1,1);
      \draw[postaction = {decorate}] (1,2)--(0.5,2.5);
      \node at (1.5,0.3) {$C$};
      \node at (1.5,2.7) {$A$};
      \node at (0.3,1.5) {$D$};
      \node at (1.5,1.5) {$S$};
      \node at (2.7,1.5) {$B$};
      \node at (1.5, 2.2) {$e_A$};
      \node at (1.5, 0.8) {$e_C$};
      \node at (2.25, 1.5) {$e_B$};
      \node at (0.75, 1.5) {$e_D$};
 \end{scope}

\begin{scope}[xshift = 4cm, scale={1},decoration={markings, mark=at
     position 0.5 with {\arrow{>}}},postaction={decorate}]
    \draw[dotted] (1.5,1.5) circle (1.414 cm);
      \draw[postaction = {decorate}] (0.5,0.5) .. controls (1,1.5) and (1,1.5) .. (0.5, 2.5);
      \draw[postaction = {decorate}] (2.5,2.5).. controls (2,1.5) and (2, 1.5) ..(2.5,0.5);  
%      \node at (1.5,0.3) {$C$};
 %     \node at (1.5,2.7) {$A$};
      \node at (0.3,1.5) {$D'$};
      \node at (1.5,1.5) {$U$};
      \node at (2.7,1.5) {$B'$};

 \end{scope}

\begin{scope}[xshift = 8cm, scale={1},decoration={markings, mark=at
     position 0.5 with {\arrow{>}}},postaction={decorate}]
    \draw[dotted] (1.5,1.5) circle (1.414 cm);
      \draw[postaction = {decorate}] (0.5,0.5) .. controls (1.5,1) and (1.5,1) .. (2.5, 0.5);
      \draw[postaction = {decorate}] (2.5,2.5).. controls (1.5,2) and (1.5,2) ..(0.5,2.5);  
      \node at (1.5,0.3) {$C''$};
      \node at (1.5,2.7) {$A''$};
%      \node at (0.3,1.5) {$D$};
      \node at (1.5,1.5) {$U$};
%      \node at (2.7,1.5) {$B$};
 \end{scope}

